Quaternion-Based Self-Attentive Long Short-Term User Preference Encoding for Recommendation

Quaternion space has brought several benefits over the traditional Euclidean space: Quaternions (i) consist of a real and three imaginary components, encouraging richer representations; (ii) utilize Hamilton product which better encodes the inter-latent interactions across multiple Quaternion components; and (iii) result in a model with smaller degrees of freedom and less prone to overfitting. Unfortunately, most of the current recommender systems rely on real-valued representations in Euclidean space to model either user's long-term or short-term interests. In this paper, we fully utilize Quaternion space to model both user's long-term and short-term preferences. We first propose a QUaternion-based self-Attentive Long term user Encoding (QUALE) to study the user's long-term intents. Then, we propose a QUaternion-based self-Attentive Short term user Encoding (QUASE) to learn the user's short-term interests. To enhance our models' capability, we propose to fuse QUALE and QUASE into one model, namely QUALSE, by using a Quaternion-based gating mechanism. We further develop Quaternion-based Adversarial learning along with the Bayesian Personalized Ranking (QABPR) to improve our model's robustness. Extensive experiments on six real-world datasets show that our fused QUALSE model outperformed 11 state-of-the-art baselines, improving 8.43% at HIT@1 and 10.27% at NDCG@1 on average compared with the best baseline.

==> 5-exp-backup.tex <==
% \vspace{-5pt}
\section{Empirical Study}
\label{sec:exp}

In this section, we design experiments to answer the following research questions:
\begin{itemize}
\item \textbf{RQ1:} How do our proposals work compared to the baselines?
\item \textbf{RQ2:} How do the user long-term, short-term preference encoding models and the fused model behave?
\item \textbf{RQ3:} Is using Quaternion representation helpful and why?
\item \textbf{RQ4:} Are the gating fusion mechanism and the Quaternion BPR adversarial training helpful?
\end{itemize}


%%%%%%%%%%%%%%%% DATASET STATISTICS %%%%%%%%%%%%%%%%%%%%
\begin{table}[t]
    \setlength\tabcolsep{1 pt}
    \centering
    \tiny
    \caption{Datasets' statistics with max \#long-term items $l$.}
    \vspace{-10pt}
    \label{table:datasets}
    \resizebox{0.88\linewidth}{!}{
        \begin{tabular}{lcccc}
            \toprule
            Dataset                      & \#users & \#items & \#actions (\% density) &   l  \\
            \midrule
            % Apps for Android            & 79,502    & 18,416    & 555,036 (0.038\%)     & 478\\
            % Cellphone Accessories       & 47,347    & 45,454    & 262,194 (0.012\%)     & 109 \\
            % % Clothing Shoes Jewelry      & 98,185    & 138,448   & 582,271 (0.004\%)     & 205 \\
            % % Digital Music               & 7,666     & 10,799    & 75,765 (0.092\%)      & \\
            % Health Care        & 53,509    & 55,759    & 363,723 (0.012\%)     & 243\\
            % Movies TV                   & 107,734   & 73,355    & 1,262,041 (0.016\%)   & 2,442\\
            % Pet Supplies                & 25,283    & 23,762    & 160,892 (0.027\%)     & 176\\
            % Sports Outdoors             & 55,477    & 67,268    & 360,501 (0.027\%)     & 328\\
            % Tools Home                  & 30,749    & 41,828    & 194,385 (0.015\%)     & 176\\
            % Toys Games                  & 36,079    & 55,641    & 251,693 (0.013\%)     & 1,112\\
            % Video Games                 & 24,429    & 20,209    & 196,661 (0.04\%)      & 856\\
            % Yelp                        & 22,015    & 21,120    & 481,284 (0.104\%)     & 930\\
            Toys Games                  & 36k    & 55k    & 251k (0.013\%)     & 1,112\\
            
            Cellphone Accessories       & 47k    & 45k    & 262k (0.012\%)     & 109 \\
            % Clothing Shoes Jewelry      & 98,185    & 138,448   & 582,271 (0.004\%)     & 205 \\
            % Digital Music               & 7,666     & 10,799    & 75,765 (0.092\%)      & \\
            % Health Care                 & 53k    & 55k    & 363k (0.012\%)     & 243\\
            % Movies TV                   & 107k   & 73k    & 1,262k (0.016\%)   & 2,442\\
            Pet Supplies                & 25k    & 23k    & 160k (0.027\%)     & 176\\
            % Sports Outdoors             & 55k    & 67k    & 360k (0.027\%)     & 328\\
            % Tools Home                  & 30k    & 41k    & 194k (0.015\%)     & 176\\
            Video Games                 & 24k    & 20k    & 196k (0.040\%)      & 856\\
            Apps for Android            & 79k    & 18k    & 555k (0.038\%)     & 478\\
            Yelp                        & 22k    & 21k    & 481k (0.104\%)     & 930\\

            \bottomrule
        \end{tabular}
    }
    \vspace{-15pt}
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%% OVERALL PERFORMANCE TABLE
% \begin{table*}[t]
% \centering
% \tiny
% \caption{Performance of the baselines, and our models. Best performances are in \emph{bold}, best baselines' results are \underline{underlined}. The last two lines show the relative improvement of QUALSE and AQUALSE compared to the best baselines' results.}
% \vspace{-10pt}
% \label{table:PerformanceComparison}
% \setlength\tabcolsep{1pt}
% \setlength\tabrowsep{1pt}
% \resizebox{1.0\textwidth}{!}{
%     \begin{tabular}{p{3.5pt}p{3.5pt} cccccccccc}
%     \toprule
% & \multicolumn{1}{c}{\multirow{2}{*}{Methods}}
% & \multicolumn{2}{c}{\textbf{Apps for Android}}
% & \multicolumn{2}{c}{\textbf{Cellphone Accessories}}
% % & \multicolumn{2}{c}{\textbf{Clothing Shoes Jewelry}}
% % & \multicolumn{2}{c}{\textbf{Digital Music}}
% & \multicolumn{2}{c}{\textbf{Health Care}}
% & \multicolumn{2}{c}{\textbf{Movies TV}}
% & \multicolumn{2}{c}{\textbf{Pet Supplies}}
% % & \multicolumn{2}{c}{\textbf{Sports Outdoors}}
% % & \multicolumn{2}{c}{\textbf{Tools Home Improvement}}
% % & \multicolumn{2}{c}{\textbf{Toys Games}}
% % & \multicolumn{2}{c}{\textbf{Video Games}}
% % & \multicolumn{2}{c}{\textbf{Yelp}}
% %& \multirow{2}{*}{\bf{RI}}
% \\
%         \cmidrule{3-12} &
%             &  HIT@100 & NDCG@100 & HIT@100 & NDCG@100 & HIT@100 & NDCG@100
%             &  HIT@100 & NDCG@100 & HIT@100 & NDCG@100
% \\
%     \midrule
% %%%%%%%%%% LONG TERM ENCODING MODEL
% \multicolumn{1}{l@{\hskip0.5pt}|}{(a)}
%             &     AASVD      &
%             0.7149 & 0.3182 & 0.5640 & 0.2443 & 0.4869 & 0.2014 & 0.6359 & 0.2637 & 0.5523 & 0.2307\\
% \multicolumn{1}{l@{\hskip0.5pt}|}{(b)}
%             &     QCF        &
%             0.6638 & 0.2864 & 0.5514 & 0.2328 & 0.4338 & 0.1821 & 0.6086 & 0.2595 & 0.5319 & 0.2194 \\
% \multicolumn{1}{l@{\hskip0.5pt}|}{(c)}
%             &     NeuMF++    &
%             0.6635 & 0.2791 & 0.5467 & 0.2291 & 0.4614 & 0.1852 & 0.5956 & 0.2502 & 0.5255 & 0.2174 \\
% \multicolumn{1}{l@{\hskip0.5pt}|}{(d)}
%             &     SASRec     &
%             0.6706 & 0.2781 & 0.5579 & 0.2239 & 0.4702 & 0.1907 & 0.6156 & 0.2562 & 0.5238 & 0.2124 \\
% \multicolumn{1}{l@{\hskip0.5pt}|}{(e)}
%             &     NAIS       &
%             0.7076 & 0.3138 & 0.5648 & 0.2427 & 0.4753 & 0.1964 & \underline{0.6369} & 0.2732 & \underline{0.5569} & 0.2302 \\

% %%%%%%%%% SHORT TERM ENCODING MODELS
% \multicolumn{1}{l@{\hskip0.5pt}|}{(f)}
%             &     FPMC       &
%             0.6659 & 0.2847 & 0.4805 & 0.1970 & 0.4024 & 0.1622 & 0.5726 & 0.2353 & 0.4405 & 0.1812 \\
% \multicolumn{1}{l@{\hskip0.5pt}|}{(g)}
%             &     AGRU       &
%             0.6969 & 0.296 & 0.5211 & 0.2030 & 0.4508 & 0.1707 & 0.5208 & 0.2030 & 0.4690 & 0.1798 \\
% \multicolumn{1}{l@{\hskip0.5pt}|}{(h)}
%             &     ALSTM      &
%             0.7043 & 0.2883 & 0.5159 & 0.2052 & 0.4361 & 0.1602 & 0.5318 & 0.2064 & 0.463 & 0.1685 \\
% \multicolumn{1}{l@{\hskip0.5pt}|}{(h)}
%             &     Caser      &
%             0.7098 & 0.3124 & \underline{0.5747} & 0.2289 & 0.4713 & 0.1880 & 0.5834 & 0.2411 & 0.4786 & 0.1859 \\

% %%%%%%%% COMBINATION OF LONG AND SHORT TERM
% % \multicolumn{1}{l@{\hskip0.5pt}|}{(i)}
% %             &     DIEN       &
% %             & & & & & & & & & \\
% \multicolumn{1}{l@{\hskip0.5pt}|}{(j)}
%             &     ALSTM+ASVD &
%             \underline{0.7173} & \underline{0.3207} & 0.5701 & \underline{0.2475} & \underline{0.4888} & \underline{0.2026} & 0.6307 & \underline{0.2775} & 0.5542 & \underline{0.2326} \\

%             \midrule
% \multicolumn{2}{l}{\textbf{Our proposed models}}
%             & & & & & & & & & \\

%             &     QUALE       &
%             0.7281 & 0.3248 & 0.6042 & 0.2685 & 0.5149 & 0.2211 & 0.6779 & 0.3021 & 0.5826 & 0.2483 \\
%             &     QUASE (GRU)         &
%             0.7198 & 0.3223 & 0.5807 & 0.2438 & 0.4789 & 0.1974 & 0.6125 & 0.2595 & 0.5413 & 0.2246 \\
%             &     QUASE (LSTM)       &
%             0.7300 & 0.3300 & 0.5844 & 0.2475 & 0.4732 & 0.1952 & 0.6144 & 0.2582 & 0.5453 & 0.2263 \\
%             &     QUALSE        &
%             \bf{0.7373} & \bf{0.3364} & \bf{0.6127} & \bf{0.2777} & \bf{0.5204} & \bf{0.2261} & \bf{0.6805} & \bf{0.3071} & \bf{0.5913} & \bf{0.2539} \\

%             \cmidrule{2-12}
%             &     AQUALE       &
%             0.7346 & 0.3306 & 0.6105 & 0.2748 & 0.5243 & 0.2286 & 0.6783 & 0.3115 & 0.5902 & 0.2553 \\

%             &     AQUASE (LSTM)      &
%             0.7285 & 0.3292 & 0.6056 & 0.2572 & 0.4907 & 0.2045 & 0.6247 & 0.2695 & 0.5520 & 0.2329 \\

%             &     AQUALSE       &
%             & & & & & & & & & \\

%             \cmidrule{2-12}

% \multicolumn{2}{l}{\textbf{Improv. of QUALSE}} &
%             \bf{+2.79\%} & \bf{+4.90\%} & \bf{+6.61\%} & \bf{+12.20\%} & \bf{+6.46\%} & \bf{+11.60\%} & \bf{+6.85\%} & \bf{+10.67\%} & \bf{+6.18\%} & \bf{+9.16\%} \\
% \multicolumn{2}{l}{\textbf{Improv. of AQUALSE }}
%             & & & & & & & & & \\
%             % & & & & & & & & & \\
%             \midrule
%             \midrule
% & \multicolumn{1}{c}{\multirow{2}{*}{}}
% & \multicolumn{2}{c}{\textbf{Sports Outdoors}}
% & \multicolumn{2}{c}{\textbf{Tools Home}}
% & \multicolumn{2}{c}{\textbf{Toys Games}}
% & \multicolumn{2}{c}{\textbf{Video Games}}
% & \multicolumn{2}{c}{\textbf{Yelp}}
% %& \multirow{2}{*}{\bf{RI}}
% \\
%         \cmidrule{3-12} &
%             &  Recall@100 & NDCG@100 & Recall@100 & NDCG@100 & Recall@100 & NDCG@100
%             &  Recall@100 & NDCG@100 & Recall@100 & NDCG@100
% \\
%     \midrule
% %%%%%%%%%% LONG TERM ENCODING MODEL
% \multicolumn{1}{l@{\hskip0.5pt}|}{(c)}
%             &     AASVD      &
%             0.5062 & 0.2137 & 0.4244 & 0.1689 & 0.4343 & 0.1809 & 0.5503 & 0.2229 & 0.7222 & \underline{0.3580}\\
% \multicolumn{1}{l@{\hskip0.5pt}|}{(a)}
%             &     QCF        &
%             0.4628 & 0.1883 & 0.3734 & 0.1455 & 0.3786 & 0.1464 & 0.5217 & 0.1956 & 0.6774 & 0.3119 \\
% \multicolumn{1}{l@{\hskip0.5pt}|}{(b)}
%             &     NeuMF++    &
%             0.4737 & 0.1904 & 0.3927 & 0.1438 & 0.3969 & 0.1553 & 0.4944 & 0.1934 & 0.681 & 0.3208 \\
% \multicolumn{1}{l@{\hskip0.5pt}|}{(d)}
%             &     SASRec     &
%             0.4825 & 0.1898 & 0.4310 & 0.1651 & 0.4009 & 0.1545 & 0.5472 & 0.2107 & 0.7193 & 0.3381 \\
% \multicolumn{1}{l@{\hskip0.5pt}|}{(e)}
%             &     NAIS       &
%             0.4850 & 0.1953 & 0.4106 & 0.1571 & 0.4276 & 0.1766 & \underline{0.5587} & 0.2303 & 0.7095 & 0.3394\\

% %%%%%%%%% SHORT TERM ENCODING MODELS
% \multicolumn{1}{l@{\hskip0.5pt}|}{(f)}
%             &     FPMC       &
%             0.4003 & 0.1600 & 0.3131 & 0.1192 & 0.337 & 0.1335 & 0.5065 & 0.1980 & 0.6704 & 0.3204 \\
% \multicolumn{1}{l@{\hskip0.5pt}|}{(g)}
%             &     AGRU       &
%             0.4361 & 0.1962 & 0.3974 & 0.1524 & 0.3747 & 0.1400 & 0.5337 & 0.1958 & 0.4722 & 0.1995 \\
% \multicolumn{1}{l@{\hskip0.5pt}|}{(h)}
%             &     ALSTM      &
%             0.4636 & 0.1815 & 0.4004 & 0.1514 & 0.3886 & 0.1419 & 0.5156 & 0.1928 & 0.5644 & 0.2519 \\
% \multicolumn{1}{l@{\hskip0.5pt}|}{(h)}
%             &     Caser      &
%             0.4629 & 0.1844 & 0.4140 & 0.1588 & 0.3889 & 0.1507 & 0.5502 & 0.1967 & 0.6718 & 0.3201 \\

% %%%%%%%% COMBINATION OF LONG AND SHORT TERM
% % \multicolumn{1}{l@{\hskip0.5pt}|}{(i)}
% %             &     DIEN       &
% %             & & & & & & & & & \\
% \multicolumn{1}{l@{\hskip0.5pt}|}{(j)}
%             &     ALSTM+ASVD &
%             \underline{0.5158} & \underline{0.2165} & \underline{0.4390} & \underline{0.1741} & \underline{0.4394} & \underline{0.1864} & 0.5502 & \underline{0.2328} & \underline{0.7277} & 0.3573  \\

%             \midrule
% \multicolumn{2}{l}{\textbf{Our proposed models}}
%             & & & & & & & & & \\

%             &     QUALE       &
%             0.5472 & 0.2344 & 0.4620 & 0.1841 & 0.4696 & 0.1997 & 0.5981 & 0.2503 & 0.7391 & 0.3723 \\
%             &     QUASE (GRU)       &
%             0.4966 & 0.2068 & 0.4134 & 0.1611 & 0.4080 & 0.1632 & 0.5612 & 0.2207 & 0.6917 & 0.3324 \\
%             &     QUASE (LSTM)       &
%             0.4970 & 0.2043 & 0.4130 & 0.1618 & 0.4095 & 0.1664 & 0.5591 & 0.2261 & 0.6929 & 0.3311 \\
%             &     QUALSE       &
%             \bf{0.5566} & \bf{0.2375} & \bf{0.4674} & \bf{0.1873} & \bf{0.4760} & \bf{0.2043} & \bf{0.6018} & \bf{0.2551} & \bf{0.7442} & \bf{0.3781} \\


%             \cmidrule{2-12}
%             &     AQUALE       &
%             0.5590 & 0.2420 & 0.4665 & 0.1875 & 0.4831 & 0.2055 & 0.6045 & 0.2593 & 0.7440 & 0.3786 \\

%             &     AQUASE (LSTM)      &
%             0.5088 & 0.2137 & 0.4365 & 0.1716 & 0.4495 & 0.1847 & 0.5762 & 0.2351 & 0.7048 & 0.3450 \\

%             &     AQUALSE       &
%             & & & & & & & & & \\

%             \cmidrule{2-12}

% \multicolumn{2}{l}{\textbf{Improv. of QUALSE}} &
%             \bf{+7.91\%} & \bf{+9.70\%} & \bf{+6.47\%} & \bf{+7.58\%} & \bf{+8.33\%} & \bf{+9.60\%} & \bf{+7.71\%} & \bf{+9.58\%} & \bf{+2.27\%} & \bf{+5.61\%} \\
% \multicolumn{2}{l}{\textbf{Improv. of AQUALSE}}
%             & & & & & & & & & \\

%             % & & & & & & & & & \\
%             \bottomrule
% \end{tabular}
% }
% \vspace{-12pt}
% \end{table*}
\begin{table*}[t]
\centering
\large
\caption{Performance of the baselines, and our models. Best performances are in \emph{bold}, best baseline's results are \underline{underlined}. The last two lines show the relative improvement of QUALSE and AQUALSE compared to the best baseline's results.}
\vspace{-10pt}
\label{table:PerformanceComparison}
\setlength\tabcolsep{0.6pt}
\resizebox{1.0\textwidth}{!}{
    \begin{tabular}{p{0.5pt}p{2pt} cccccccccccc}
    \toprule
& \multicolumn{1}{c}{\multirow{2}{*}{Methods}}
& \multicolumn{2}{c}{\textbf{Toys Games}}
& \multicolumn{2}{c}{\textbf{Cellphone Accessories}}
% & \multicolumn{2}{c}{\textbf{Clothing Shoes Jewelry}}
% & \multicolumn{2}{c}{\textbf{Digital Music}}
% & \multicolumn{2}{c}{\textbf{Health Care}}
% & \multicolumn{2}{c}{\textbf{Movies TV}}
& \multicolumn{2}{c}{\textbf{Pet Supplies}}
% & \multicolumn{2}{c}{\textbf{Sports Outdoors}}
% & \multicolumn{2}{c}{\textbf{Tools Home Improvement}}
& \multicolumn{2}{c}{\textbf{Video Games}}
& \multicolumn{2}{c}{\textbf{Apps for Android}}
& \multicolumn{2}{c}{\textbf{Yelp}}
%& \multirow{2}{*}{\bf{RI}}
\\
        \cmidrule{3-14} &
            & Hit@100 & NDCG@100
            & Hit@100 & NDCG@100
            & Hit@100 & NDCG@100
            & Hit@100 & NDCG@100
            & Hit@100 & NDCG@100
            & Hit@100 & NDCG@100
\\
    \midrule
%%%%%%%%%% LONG TERM ENCODING MODEL
\multicolumn{1}{l@{\hskip0.5pt}|}{(a)}
            &     AASVD      &
            0.4343 & 0.1809 & 0.5640 & 0.2443 & 0.5523 & 0.2307
            & 0.5503 & 0.2229 & 0.7149 & 0.3182 
            & 0.7212 & 0.3580\\
\multicolumn{1}{l@{\hskip0.5pt}|}{(b)}
            &     QCF        &
            0.3869 & 0.1560 & 0.5514 & 0.2328 & 0.5319 & 0.2194
            & 0.5217 & 0.1956 & 0.6638 & 0.2864 
            & 0.6774 & 0.3119
            \\
\multicolumn{1}{l@{\hskip0.5pt}|}{(c)}
            &     NeuMF++    &
            0.3969 & 0.1553 & 0.5467 & 0.2291 & 0.5255 & 0.2174
            & 0.4944 & 0.1934 & 0.6635 & 0.2791 
            & 0.6810 & 0.3208\\

\multicolumn{1}{l@{\hskip0.5pt}|}{(d)}
            &     NAIS       &
            0.4331 & 0.1796 & 0.5648 & 0.2427 & \underline{0.5569} & 0.2302
            & \underline{0.5587} & 0.2303 & 0.7076 & 0.3138 & \underline{0.7277} & 0.3573 \\

%%%%%%%%% SHORT TERM ENCODING MODELS
\multicolumn{1}{l@{\hskip0.5pt}|}{(e)}
            &     FPMC       &
            0.3370 & 0.1335 & 0.4805 & 0.1970 & 0.4405 & 0.1812
            & 0.5065 & 0.1980 & 0.6659 & 0.2847 
            & 0.6704 & 0.3204\\
\multicolumn{1}{l@{\hskip0.5pt}|}{(f)}
            &     AGRU       &
            0.3747 & 0.1400 & 0.5211 & 0.2030 & 0.4690 & 0.1798
            & 0.5337 & 0.1958 & 0.6969 & 0.2960 
            & 0.4722 & 0.1995\\
\multicolumn{1}{l@{\hskip0.5pt}|}{(g)}
            &     ALSTM      &
            0.3886 & 0.1419 & 0.5159 & 0.2052 & 0.4630 & 0.1685
            & 0.5156 & 0.1928 & 0.7043 & 0.2883 & 
            0.5644 & 0.2519 \\
\multicolumn{1}{l@{\hskip0.5pt}|}{(h)}
            &     Caser      &
            0.3889 & 0.1507 & \underline{0.5747} & 0.2289
            & 0.4786 & 0.1859
            &  0.5502 & 0.1967 & 0.7098 & 0.3124 &
            0.6718 & 0.3201\\

%%%%%%%% COMBINATION OF LONG AND SHORT TERM
% \multicolumn{1}{l@{\hskip0.5pt}|}{(i)}
%             &     DIEN       &
%             & & & & & & & & & \\

\multicolumn{1}{l@{\hskip0.5pt}|}{(i)}
            &     SASRec     &
            0.4009 & 0.1545 & 0.5579 & 0.2239 & 0.5238 & 0.2124
            & 0.5472 & 0.2107 & 0.6706 & 0.2781 & 0.7193 & 0.3381\\
            
\multicolumn{1}{l@{\hskip0.5pt}|}{(j)}
            &     \text{SLi-Rec} &
            0.4267 & 0.1823 & 0.5661 & 0.2387 & 0.5502 & 0.2311
            & 0.5438 & 0.2276 & 0.7062 & 0.3117 &  0.7201 & 0.3516\\
            
\multicolumn{1}{l@{\hskip0.5pt}|}{(k)}
            &     ALSTM+AASVD &
            \underline{0.4394} & \underline{0.1864} & 0.5701 & \underline{0.2475} & 0.5542 & \underline{0.2326}
            & 0.5502 & \underline{0.2328} & \underline{0.7173} & \underline{0.3207} &  {0.7222} & \underline{0.3594}\\

            \midrule
\multicolumn{2}{l}{\textbf{Our proposals}}
            & & & & & & & & & & & \\

            &     QUALE       &
            0.4696 & 0.1997 & 0.6042 & 0.2685 & 0.5826 & 0.2483
            & 0.5981 & 0.2503 & 0.7281 & 0.3248 & 0.7391 & 0.3723\\
            &     QUASE\;(GRU)         &
            0.4080 & 0.1632 & 0.5612 & 0.5807 & 0.2438 & 0.5413 & 0.2246
            & 0.2207 & 0.7198 & 0.3223 & 0.6917 & 0.3324\\
            &     QUASE\;(LSTM)       &
            0.4095 & 0.1664 & 0.5844 & 0.2475 & 0.5453 & 0.2263
            & 0.5591 & 0.2261 & 0.7300 & 0.3300 & 0.6929 & 0.3311\\
            &     QUALSE        &
            \bf{0.4760} & \bf{0.2043} & \bf{0.6127} & \bf{0.2777} & \bf{0.5913} & \bf{0.2539}
            & \bf{0.6018} & \bf{0.2551} & \bf{0.7373} & \bf{0.3364} & \bf{0.7442} & \bf{0.3781}\\

            \cmidrule{2-14}
            &     AQUALE       &
            0.4831 & 0.2055 & 0.6105 & 0.2748 & 0.5902 & 0.2553
            & 0.6045 & 0.2593 & 0.7346 & 0.3306 & 0.7440 & 0.3786\\

            &     AQUASE\;(LSTM)      &
            0.4495 & 0.1847 & 0.6056 & 0.2572 & 0.5520 & 0.2329
            & 0.5762 & 0.2351 & 0.7285 & 0.3292 & 0.7048 & 0.3450 \\

            &     AQUALSE       &
            \bf{0.4921}	& \bf{0.2098}  & \bf{0.6204} & \bf{0.2842} & \bf{0.6011}  & \bf{0.2612} & \bf{0.6137} & \bf{0.2605} & \bf{0.7477} & \bf{0.3440} & \bf{0.7448} & \bf{0.3814} \\

            \cmidrule{2-14}

\multicolumn{2}{l}{\textbf{Imprv. of QUALSE}} &
            \bf{+8.33\%} & \bf{+9.60\%} &
            \bf{+6.61\%} & \bf{+12.20\%} &
            \bf{+6.18\%} & \bf{+9.16\%} &
            \bf{+7.71\%} & \bf{+9.58\%} &
            \bf{+2.79\%} & \bf{+4.90\%} &
            \bf{+2.27\%} & \bf{+5.20\%}\\
\multicolumn{2}{l}{\textbf{Imprv. of AQUALSE }}
            & \bf{+11.99\%} & \bf{+12.55\%}
            & \bf{+7.95\%} & \bf{+14.83\%}
            & \bf{+7.94\%} & \bf{+12.30\%}
            &  \bf{+9.84\%} & \bf{+11.90\%}
            & \bf{+4.24\%} & \bf{+7.27\%}
            & \bf{+2.35\%} & \bf{+6.12\%} \\
            % & & & & & & & & & \\
\bottomrule
\end{tabular}
}
\vspace{-12pt}
\end{table*}
%%%%%%%%%%%%%% END OVERALL PERFORMANCE TABLE


\subsection{Datasets}
We evaluate all models on \textbf{six} public datasets from two real world systems as follows:
%\begin{itemize}
\squishlist
    %\item {\bf Amazon} \cite{he2016ups}: A series of datasets crawled from \emph{Amazon.com}. We use 9 different categories: \emph{Apps for Android}, \emph{Cellphone Accessories}, \emph{Health \& Personal Care}, \emph{Movies TV}, \emph{Pet Supplies}, \emph{Sports \& Outdoors}, \emph{Tools and Home Improvement}, \emph{Toys and Games}, and \emph{Video Games}.
    \item {\bf Amazon datasets}: We use 5 different Amazon category datasets from \cite{he2016ups}: \emph{Apps for Android}, \emph{Cellphone Accessories}, \emph{Pet Supplies}, \emph{Toys and Games}, and \emph{Video Games}. These categories are selected as to promote sparsity, variability, and data size.
    \item {\bf Yelp dataset}: This is a user rating dataset on businesses. We use the dataset from \cite{he2016fast}.%, where repetitive user-item interactions are merged to the earliest one to avoid training interactions appearing in the test set.
%\end{itemize}
\squishend

For data preprocessing, we adopted a widely-used \emph{k-core} preprocessing step \cite{he2016ups} (with $k$=5), filtering out users and items with less than 5 interactions. All observed ratings are considered as positive interactions and the remaining as negative interactions. The maximum number of short-term items is set to $s=5$ in all datasets as it covers the short-term peak (Figure \ref{fig:train_stat}). In long term, we observe that several users in Amazon datasets consumed an extremely large number of items compared to the majority of users. It will cost large amount of unnecessary zero paddings if we decide to cover all these outlier users. %To select the maximum number of long-term items $l$, we observe that several users in Amazon datasets consumed an extremely large number of items compared to the majority of users. If we consider those extreme users, majority of users' historical items will be unnecessarily padded zeroes.
Hence, we set $l$ to the upper bound of the boxplot approach (i.e. Q3 + 1.5IQR, where Q3 is the \emph{third quartile}, and IQR is the \emph{Interquartile range} of the sequence length distribution of all users). Table \ref{table:datasets} summarizes the statistics of all datasets.

\vspace{-10pt}
\subsection{State-of-the-art Baselines}
We compared our proposed models with \textbf{11} strong state-of-the-art recommendation models as follows:
%\begin{itemize}
\squishlist
    \item {\bf AASVD}: It is an attentive version of the well-known Asymmetric SVD model (ASVD) \cite{koren2008factorization},
    where real-valued self-attention is applied to measure attentive contribution of past items.

    %In ASVD, users are represented by averaging their consumed items' latent representations equally. AASVD extends ASVD by measuring attentive contribution of consumed items. %Note that AASVD uses the same self-attention with our proposed QAASVD, where Hamilton products and Quaternion embeddings are replaced by dot product and real-valued embeddings.
    \item {\bf QCF} \cite{zhang2019quaternion}: It is a recent state-of-the-art recommender that represents users/items by Quaternion embeddings.
    \item {\bf NeuMF++} \cite{he2017neural}: It is a state-of-the-art neural recommender that models non-linear user-item interactions by using a MLP and a Generalized MF (GMF) component. We pretrain MLP and GMF to obtain NeuMF's best performance.
    \item {\bf NAIS} \cite{he2018nais}: It is an extension of \emph{ASVD} where contribution of consumed items to the target item are attentively assigned. We adopt $NAIS_{prod}$ version as it led to its best results.
    \item {\bf FPMC} \cite{rendle2010factorizing}: It is a state-of-the-art sequential recommender. It uses the first-order Markov to model the transition between the next item and the previously consumed items.
    \item {\bf AGRU}: It is an extension of the well-known GRU4Rec \cite{hidasi2015session}, where we use an attention mechanism to combine different hidden states. We experiment with two attention mechanisms: real-valued self-attention, and real-valued \emph{prod attention} proposed by \cite{he2018nais}. Then we report its best performance.
    \item {\bf ALSTM}: It is a LSTM based model. Similar to AGRU, we experiment with the real-valued self-attention and the \emph{prod attention} \cite{he2018nais}, then report its best results.
    \item {\bf Caser} \cite{tang2018personalized}: It is a widely used sequential recommender. %It uses convolution neural network design.
    It embedded a sequence of recently consumed items into an ``image'' in time and latent spaces and uses convolution neural network to learn sequential patterns as local features of an image using different horizontal and vertical filters.
     \item {\bf SASRec} \cite{kang2018self}: It is a strong sequential recommender model. It uses the self-attention mechanism with a multi-head design to identify relevant items for next predictive items.
    \item \textbf{Sli-Rec} \cite{yu2019adaptive}: It uses a time-aware controller to control the state transition, then use an attention-based framework to fuse users long-term and short-term preferences.
    \item {\bf ALSTM+AASVD}: It is our implementation. It resembles a same architecture as our Quaternion fusion proposals, except that it uses Euclidean space instead of Quaternion space.
    %incorporating estimated
    %learning both long-term and short-term user interests.
%\end{itemize}
\squishend

First four baselines (AASVD, QCF, NeuMF++, NAIS) are classified as user's long-term interest encoding models. Next four baselines (FPMC, AGRU, ALSTM, Caser) are user's short-term interest encoding models, and \emph{SASRec, SLi-Rec, ALSTM+AASVD} encodes both user long and short-term intents.
Note that we performed experiment with \emph{DIEN} \cite{zhou2019deep} (i.e. a long short-term modeling baseline) based on the authors' public source code, but we got surprisingly low results so we omit its detailed results.
% Note that we also experimented ASVD \cite{koren2008factorization}, LSTM, GRU, Quaternion LSTM \cite{parcollet2018quaternion}, SLIM \cite{ning2011slim}, FISM \cite{kabbur2013fism}, MF-BPR, but do not report their results due to space limitation and their worse results compared to the above baselines.
We also experimented with \emph{ASVD}, LSTM, GRU and Quaternion LSTM but do not report their results due to space limitation and their worse results. Similarly, we omit \emph{BPR} \cite{rendle2012bpr} and \emph{FISM} \cite{kabbur2013fism} results due to their less impressive results.
%We do not report \emph{BPR} because NeuMF++ outperformed it. Similarly, \emph{NAIS} outperformed \emph{SLIM} \cite{ning2011slim}, \emph{FISM} \cite{kabbur2013fism} so we do not report their results.

% We compare the above baselines with our proposals as follows:
% \squishlist
%     \item {\bf QUALE}: Our proposal to model users' long-term preferences.
%     \item {\bf QUASE (GRU/LSTM)}: Our proposal to model users' short-term preferences using the Quaternion self-attentive GRU/LSTM.
%     \item {\bf QUALSE}: Our fusion to model both user's long-term and short-term preferences.
%     \item {\bf AQUALE}: Our Adversarial QUALE model, learning with our proposed Quaternion adversarial learning.
%     \item {\bf AQUASE}: Our Adversarial QUASE model.
%     \item {\bf AQUALSE}: Our Adversarial fused QUALSE model.
    
    
\squishend
% \vspace{-5pt}
\subsection{Experimental Settings}
\noindent\textbf{Protocol}: We adopt a well-known and practical 70/10/20 splitting proportions to divide each dataset into train/validation (or development)/test sets \cite{liang2016modeling,wang2019neural,liang2018variational}. All user-item interactions are sorted in ascending order in terms of the interaction time. Then, the first 70\% of all interactions are used for training, the next 10\% of all interactions are used for development, and the rest is used for testing. We follow \cite{wang2019neural,xin2019relational} to sample 1,000 unobserved items that the target user has not interacted before and rank all her positive items with these 1,000 unobserved items for testing models.

\noindent\textbf{Evaluation metrics:} We evaluate the performances of all models by using two well-known metrics: \emph{Recall} or \emph{Hit} Ratio (\emph{HIT@N}), and Normalized Discounted Cumulative Gain (\emph{NDCG@N}). \emph{HIT@N} measures whether all the test items are in the recommended list or not, while \emph{NDCG@N} takes into account the position of the test items and assign higher scores if test items are at top-rank positions.

\noindent\textbf{Hyper-parameters Settings:} All models are trained with \emph{Adam} optimizer \cite{kingma2014adam}. Learning rate is chosen from \{0.001, 0.0005\}, regularization hyperparamters are chose from \{0, 0.1, 0.001, 0.000001\}. Embedding size $d$ are from \{32, 48, 64, 96, 128\}. Note that for Quaternion embeddings, each component value is a vector of size $\frac{d}{4}$. The number of epochs is 30. The batch size is 256. The number of MLP layers in NeuMF++ is tuned from \{1, 2, 3\}. The number of negative samples per one positive instance is 4 for training models. The settings of \emph{Caser}, \emph{NAIS}, \emph{SASRec} are followed by their reported default settings. In training with \emph{QABPR} loss, the regularization $\lambda_{adv}$ is set to 1. The noise magnitude $\epsilon$ is chose from \{0.5, 1, 2\}. The adversarial noise is added only in training process, and is initialized as \emph{zero}. All hyper-parameters are tuned by using the development set.

% \vspace{-10pt}
\subsection{Experimental Results}
%Table \ref{table:PerformanceComparison} shows the performances of our models and all the compared baselines on six datasets. We use the results to answer the following research questions:

\noindent\textbf{RQ1: Our models vs baselines?} Table \ref{table:PerformanceComparison} shows that our proposed fused models \emph{QUALSE}
%(i.e. training with \emph{BPR} loss)
and \emph{AQUALSE}
%(i.e. \emph{QUALSE} but training with our \emph{QABPR} loss)
outperformed all the compared baselines. On average, \emph{QUALSE} improved \emph{Hit@100} by 5.65\% and \emph{NDCG@100} by 8.44\% compared to the best baseline's performances. \emph{AQUALSE} gains additional improvement compared to \emph{QUALSE}, enhancing \emph{Hit@100} by 7.39\% and \emph{NDCG@100} by 10.83\% on average compared to the best baseline's performances. The improvement of our proposed models over the baselines is significant under the Directional Wilcoxon signed-rank test (\emph{p-value} $< 0.015$).

To further confirm the effectiveness of our proposals, we compare QUALSE and AQUALSE models with the top-5 baselines when varying the embedding size from \{32, 48, 64, 96, 128\} and the \emph{topN} recommendation list from \{10, 20, 50, 100\}. %The results are shown in Figure \ref{fig:sensitivity-topN-embedsize}. 

Figure \ref{fig:video-game-varyTopN-ndcg} shows that even with small \emph{topN} values, our models consistently outperformed all the compared baselines in the Video Games dataset, improving the ranking performance by a large margin of 9.25\%$\sim$12.30\% on average. Specifically, at \emph{topN}=10 in Video Games dataset, QUALSE and AQUALSE improves NDCG@10 over the best baseline by 9.9\% and 12.97\%, respectively. Even with \emph{topN=1}, we also observe similar results on all six datasets. On average over six datasets, our proposals improved HIT@1 and NDCG@1 by 8.6\% compared to the best baseline. 

Figure \ref{fig:yelp-vary-embed-hit} shows the HIT@100 performance of our QUALSE, AQUALSE models, and the top-5 baselines in the Yelp dataset when varying the embdding size from \{32, 48, 64, 96, 128\}. We observe that our proposals outperformed all the baselines. Interestingly, while non-adversarial models are more sensitive to the change of the embedding size, our adversarial AQUALSE model is smoother when varying the embedding size. This is obvious, as the goal of the adversarial learning is to reduce the noise effect, and so does our proposed Quaternion adversarial training method.  

% \noindent\textbf{Sensitivity of our Quaternion-based proposals when varying \emph{top-N} recommendation list and embedding size?} We show the NDCG performances of our \emph{QUALSE}, \emph{AQUALSE} and the best five baselines when varying the \emph{top-N} recommendation list from \{10, 20, 50, 100\} (Figure \ref{fig:video-game-varyTopN-ndcg}) on Video Games dataset, and when varying the embedding size from \{32, 48, 64, 96, 128\} (Figure \ref{fig:yelp-vary-embed-ndcg}) in Yelp dataset. We observe that our proposals perform better than the best five baselines. Particularly, on average, \emph{QUALSE} improves \emph{NDCG} by 2.45$\sim$7.52\%, and  \emph{AQUALSE} improves \emph{NDCG} by 4.66$\sim$8.84\% compared to the best baseline performances.


%%%%%%%%%% VARY TOP-N figures
\begin{figure}[t]
    \includegraphics[width=0.42\textwidth]{figs/vary-topN-legend2.pdf}
    \centering
	\begin{subfigure}{0.23\textwidth}
		\centering
		\includegraphics[width=\textwidth]{figs/NDCG-VideoGames2.jpeg}
		\vspace{-10pt}
		\caption{NDCG@topN in Video Games}
		\label{fig:video-game-varyTopN-ndcg}
	\end{subfigure}
	\begin{subfigure}{0.23\textwidth}
		\centering
		\includegraphics[width=\textwidth]{figs/HIT-yelp2.jpeg}
		\vspace{-10pt}
		\caption{HIT@100 in Yelp.}
		\label{fig:yelp-vary-embed-hit}
	\end{subfigure}
    \vspace{-10pt}
    \caption{Performance of our models and the baselines when varying \emph{top-N} recommendation list from \{10, 20, 50, 100\} (left) and embedding size from \{32, 48, 64, 128\} (right). %Five best baselines are compared with \emph{QUALSE} and \emph{AQUALSE} for a clear visualization.
    }
    \label{fig:sensitivity-topN-embedsize}
    \vspace{-15pt}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\noindent\textbf{RQ2: Long-term vs short-term vs fused models?} 
Using reported results in Table \ref{table:PerformanceComparison}, we first compare long-term encoding models (i.e. (a)-(d), and \emph{QUALE}, \emph{AQUALE}) vs with short-term encoding models (i.e. (e)-(h), and \emph{QUASE}, \emph{AQUASE}). In general, long-term encoding models work better than short-term encoding models. For instance, NAIS (i.e. best long-term encoding baseline) improves 8.5\% on average on six datases compared with Caser (i.e. best short-term encoding baseline). Similarly, our long-term encoding \emph{QUALE} model works better than our short-term encoding \emph{QUASE} model, enhancing 9.2\% on average over six datasets. To investigate this phenomenon, we plot the density distribution of item-item similarity scores for two datasets \emph{Pet-Supplies} and \emph{Yelp} in Figure \ref{fig:density-exp}. We observe higher peaks on long-term item-item relationships in the testing curve (i.e. the green curve), explaining why long-term encoding models work better than short-term encoding models. 

Next, we compare the fused models with models that encode either long-term or short-term users preferences. Table \ref{table:PerformanceComparison} shows that models that consider both user long-term and short-term preferences work better than models that encode either user long-term or short-term interests. Both (j) and (k) baselines generally work better than (a)--(h) baselines. Specifically, our QUALSE and AQUALSE models improve 7.9\%$\sim$10.0\% on average over six datasets compared to the best baseline from (a)--(h). These observations show the effectiveness of modelling both user long-term and short-term interests. 
Among models that consider both user long-term and short-term interests, SASRec performed worst compared to baselines (i)--(k) and our QUALSE and AQUALSE. This is due to the fact that SASRec models user long-term and short-term interests implicitly and concurrently using the Transformer multi-head attention mechanism, whereas SLi-Rec, ALSTM+AASVD, and our proposals model the two preferences explicitly and separately and then combine them later on, which encourage more flexibility. Note that, although SLi-Rec employed a time-aware attentional LSTM to better model the user short-term preferences, our ALSTM+AASVD implementation works slightly better than SLi-Rec due to its two distinct properties: (i) the personalized self-attention in AASVD, where each user is parameterized by her own context vector, and (ii) the personalized gating fusion. To further confirm, we experiment that without using the personalized self-attention (i.e. use a single global context vector for all users), performance of AASVD and \emph{QUALE} drop by 3.12\% on average over six datasets. Without the personalized gating fusion, performance of ALSTM+AASVD and \emph{QUALSE} drop by 2.29\% on average over six datasets.   

\noindent\textbf{RQ3: Is using Quaternion representation helpful?} In Table \ref{table:PerformanceComparison}, we compare different model pairs: \emph{AASVD} vs. \emph{QUALE}, \emph{ALSTM} vs. \emph{QUASE (LSTM)}, \emph{AGRU} vs. \emph{QUASE (GRU)}, and \emph{ALSTM+AASVD} vs. \emph{QUALSE}. Note that \emph{AASVD} shares exactly the same architecture with \emph{QUALE}, except that \emph{QUALE} uses Quaternion representations, while \emph{AASVD} uses real-valued representations, and so do the other pairs. Table \ref{table:PerformanceComparison} shows that \emph{QUALE} works better than \emph{AASVD}. %For example, in \emph{Cellphone Accessories} dataset, \emph{QUALE} enhances \emph{AASVD} by 7.47\% of \emph{Hit@100} and 12.20\% of \emph{NDCG@100}. In \emph{Video Games} dataset, \emph{QUALE} improves \emph{AASVD} by 9.38\% of \emph{Hit@100} and 9.58\% of \emph{NDCG@100}.
In six datasets, on average, \emph{QUALE} improves \emph{Hit@100} by 5.60\% and \emph{NDCG@100} by 7.71\% compared to \emph{AASVD} model. Similarly, we observe the same patterns from the other three model pairs. %for other comparisons of pairs of models, we observe that in six datasets, on average, \emph{QUASE (LSTM)} improves \emph{ALSTM} by 11.88\% of \emph{Hit@100} and 22.56\% of \emph{NDCG@100}; \emph{QUASE (GRU)} boosts \emph{AGRU} by 15.11\% of \emph{Hit@100} and 24.97\% of \emph{NDCG@100}; \emph{QUALSE} enhances \emph{ALSTM+ASVD} by 6.16\% of \emph{Hit@100} and 8.54\% of \emph{NDCG@100}.
Moreover, when comparing our long-term encoding \emph{QUALE} and \emph{AQUALE} models with other long-term encoding baselines (a)-(e), our models outperformed the baselines, improving \emph{HIT@100} by 5.16\% and 6.55\%, and enhancing \emph{NDCG@100} by 7.11\% and 9.83\%, respectively. %On average six datasets, \emph{QUALE} improves \emph{HIT@100} by 5.16\% and \emph{NDCG@100} by 7.11\% compared to the best long-term baselines (a)-(e) (\emph{p-value} $< 0.05$), while \emph{AQUALE} improves \emph{HIT@100} by 6.55\% and \emph{NDCG@100} by 9.83\% compared to the best long-term baselines (a)-(e) (\emph{p-value} $< 0.015$).
Similarly, our short-term encoding \emph{QUASE} and \emph{AQUASE} using LSTM also work better than other short-term encoding baselines (f)-(h), improving \emph{HIT@100} by 4.75\% and 8.09\%, and enhancing \emph{NDCG@100} by 10.57\% and 15.33\%, respectively.
%We note that performance of \emph{QUASE} when using Quaternion LSTM is slightly better (+0.97\%) than Quaternion GRU, which is consistent to results of real-valued LSTM and real-valued GRU in the literature \cite{cho2014learning}.
All of these results confirm the effectiveness of modeling user's interests by using Quaternion representations over traditional real-valued representations.

\noindent\textbf{Why Quaternion representations help improve the performance?} Since attention mechanism is the key success in deep neural networks \cite{vaswani2017attention}, we analyze how our models assign attention weights compared to their respective real-valued models. We first measure the item-item Pointwise Mutual Information%\footnote{https://en.wikipedia.org/wiki/Pointwise\_mutual\_information} 
(PMI) scores (i.e. $PMI(k,t) = log \frac{P(k,t)}{P(k)\times P(t)}$) using the training set. The PMI score between two items ($k, t$) gives us the co-occurrence information between item $k$ and $t$, or how likely the target item $k$ will be preferred by the target user when the item $t$ is already in her consumed item list. We perform \emph{softmax} on all item-item PMI scores. Then we compare with the generated attention scores from our proposed models and their respective real-valued baseline models. We show the scatter plots and Pearson correlation comparison in Figure \ref{fig:attention-analysis}. We see that \emph{QUALE, QUASE} tend to correlate more positively with the PMI scores than their respective real-valued models \emph{AASVD, ALSTM}. In another word, our Quaternion-based models assign higher scores for co-occurred item pairs, in which we reason coming from two aspects of Quaternion representations. First, Hamilton product in Quaternion space encourages strong inter-latent interactions across Quaternion components. Second, since our proposed self-attention mechanism produces scores in Quaternion space, the output attention scores have four values \emph{w.r.t} four Quaternion components. This can be thought as similar to the multi-head attention mechanism \cite{vaswani2017attention} (but not exactly same because of the weight shared in Quaternion transformation), where the proposed attention mechanism learns to attend different aspects from the four Quaternion components. All of these explain why we get better results compared to the respective real-valued models.



\noindent\textbf{RQ4: Is adaptively fusing long-term and short-term user interests helpful?}
Table \ref{table:PerformanceComparison} shows that in real-valued representations, \emph{ALSTM+ASVD} works better than \emph{AASVD} and \emph{ALSTM} in all six datasets. %Particularly, in \emph{Toys and Games}, \emph{ALSTM+ASVD} improves \emph{Hit@100} by 1.17\% and \emph{NDCG@100} by 3.04\%  compared to the best performances of \emph{AASVD} and \emph{ALSTM}.
%On average, in six datasets, \emph{ALSTM+ASVD} improves 1.2\% performance compared to the best results of its two degenerated models. 
Similarly, in Quaternion representations, the fused \emph{QUALSE} model
%(i.e. fusion of \emph{QUALE} and \emph{QUASE} with LSTM cell)
generally works better than its two degenerated \emph{QUALE} and \emph{QUASE} models. %For instance, \emph{QUALSE} enhances \emph{Hit@100} by 1.41\%  and \emph{NDCG@100} by 3.43\% in \emph{Cellphone Accessories} dataset compared to the best results of its two degenerated models.
% In six datasets, \emph{QUALSE} performs 1.7\% better than the maximum performances of its two degenerated models. %Additionally, \emph{AQUALSE} also works better than \emph{AQUALE} and \emph{AQUASE}, improving \emph{Hit@100} by 1.46\%  and \emph{NDCG@100} by 2.18\% on average compared to the best performances of \emph{AQUALE} and \emph{AQUASE}.
% Additionally, \emph{AQUALSE} also works 1.82\% better than the maximum performances of \emph{AQUALE} and \emph{AQUASE}. 
In six datasets, both \emph{QUALSE} and \emph{AQUALSE} performs better than their degenerated (adversarial) versions, improving 2\% on average \emph{w.r.t} both \emph{HIT@100} and \emph{NDCG@100}. %Additionally, \emph{AQUALSE} also works better than \emph{AQUALE} and \emph{AQUASE}, improving \emph{Hit@100} by 1.46\%  and \emph{NDCG@100} by 2.18\% on average compared to the best performances of \emph{AQUALE} and \emph{AQUASE}.
% Additionally, \emph{AQUALSE} also works 1.82\% better than the maximum performances of \emph{AQUALE} and \emph{AQUASE}. 
Though the results confirm the effectiveness of fusing long-term and short-term user preferences in both of \emph{QUALSE} and \emph{AQUALSE}, their improvements are not highly boosted. To investigate the reason, we observe the density distribution of item-item similarity scores by using the training, validation and test sets, separately.





% %%%%%%%%%% VARY embedding size
% \begin{figure}[t]
%     \includegraphics[width=0.42\textwidth]{figs/vary-topN-legend.pdf}
%     \centering
% 	\begin{subfigure}{0.2\textwidth}
% 		\centering
% 		\includegraphics[width=\textwidth]{figs/yelp-hits-varyembedding.pdf}
% 		\vspace{-10pt}
% 		\caption{HIT@topN}
% 		\label{fig:yelp-varyembed-hit}
% 	\end{subfigure}
% 	\begin{subfigure}{0.2\textwidth}
% 		\centering
% 		\includegraphics[width=\textwidth]{figs/yelp-ndcg-varyembedding.pdf}
% 		\vspace{-10pt}
% 		\caption{NDCG@topN.}
% 		\label{fig:yelp-varyembed-ndcg}
% 	\end{subfigure}
%     \vspace{-10pt}
%     \caption{Performance of our best models \emph{QUALSE} and \emph{AQUALSE} against top-5 baselines when varying embedding size from \{32, 48, 64, 96, 128\} on Yelp dataset.} %Five best baselines are compared with \emph{QUALSE} and \emph{AQUALSE} for a clear visualization.}
%     \label{fig:vary-embedding}
%     \vspace{-15pt}
% \end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \noindent\textbf{Sensitivity of our Quaternion-based proposals when varying \emph{top-N} recommendation list and embedding size?} We show the NDCG performances of our \emph{QUALSE}, \emph{AQUALSE} and the best five baselines when varying the \emph{top-N} recommendation list from \{10, 20, 50, 100\} (Figure \ref{fig:video-game-varyTopN-ndcg}) on Video Games dataset, and when varying the embedding size from \{32, 48, 64, 96, 128\} (Figure \ref{fig:yelp-vary-embed-ndcg}) in Yelp dataset. We observe that our proposals perform better than the best five baselines. Particularly, on average, \emph{QUALSE} improves \emph{NDCG} by 2.45$\sim$7.52\%, and  \emph{AQUALSE} improves \emph{NDCG} by 4.66$\sim$8.84\% compared to the best baseline performances.
%Figure \ref{fig:varytopN-video-game} shows performances of our \emph{QUALSE}, \emph{AQUALSE} and the best five baselines when varying the \emph{top-N} recommendation list from \{10, 20, 50, 100\} and 

%. We observe that all models gain better results when increasing the \emph{top-N} and our proposals perform better than the best five baselines in all \emph{top-N} experiments. Particularly, on average \emph{QUALSE} improves \emph{Hit}@\emph{top-N} by 5.32\%, \emph{NDCG@top-N} by 7.52\% compared to the best baseline performances. \emph{AQUALSE} additionally boost \emph{QUALSE} with \emph{QABPR} loss, improving \emph{Hit}@\emph{top-N} by 5.88\%, \emph{NDCG@top-N} by 8.84\% compared to the best baseline performances. %Again, the \emph{HIT} improvement of \emph{AQUALSE} over \emph{QUALSE} is not as high as with \emph{NDCG} since \emph{QABPR} loss operates on the \emph{BPR} loss, which aims on improving ranking of positive items over negative items.
%Figure \ref{fig:vary-embedding} shows the \emph{HIT@100} and \emph{NDCG@100} performances of our best proposals \emph{QUALSE} and \emph{AQUALSE} versus the best five baselines when varying the embedding size from \{32, 48, 64, 96, 128\}. Overall, on average, \emph{QUALSE} improves 2.45\% and \emph{AQUALSE} improve 4.66\% on both \emph{HIT@100} and \emph{NDCG@100} compared to the best baseline's performance.



%%%%%%%%%% DENSITY SCORES
\begin{figure}[t]
    \includegraphics[width=0.42\textwidth]{figs/density_legend.png}
    \centering
    \begin{subfigure}{0.22\textwidth}
		\centering
		\includegraphics[width=\textwidth, height=60pt]{figs/pet_density.pdf}
		\vspace{-10pt}
		\caption{Pet Supplies dataset.}
		\label{fig:density-exp-pet}
	\end{subfigure}
    \begin{subfigure}{0.22\textwidth}
		\centering
		\includegraphics[width=\textwidth, height=60pt]{figs/yelp_density.pdf}
		\vspace{-10pt}
		\caption{Yelp dataset.}
		\label{fig:density-exp-yelp}
	\end{subfigure}
	\vspace{-10pt}
    \caption{Density distribution of item-item similarity scores on Pet and Yelp. Best viewed in colors.}
    \label{fig:density-exp}
    \vspace{-15pt}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Figure \ref{fig:density-exp} shows the density distribution of item-item similarity scores on \emph{Pet Supplies} and \emph{Yelp} dataset. The training set of each of both datasets  (i.e. blue curve) has two peaks. The left peak (i.e. short-term item dependencies) is much higher than the right peak (i.e. long-term item dependencies), indicating that target items in the training set tend relate more to recently consumed items, rather than items that were consumed long time ago. Unfortunately, in the validation and test sets, we observe a higher peak on the long-term consumed items, showing a stronger long-term item-item relationships. This mismatch explains not only the small improvements of our fused models over our degenerated models, but also the higher results of long-term user encoding model compared to the short-term user encoding model we have reported in Table \ref{table:PerformanceComparison}.

We further compare our gating fusion mechanism with a weight fixing method, where we assign a contribution score $c \in [0, 1]$ for the user short-term preference encoding part and $1-c$ for the long-term part. We see that the gating fusion improves 4.82\% on average over six datasets compared to the weight fixing method. It makes sense, as the weight fixing method assumes a same contribution rate of the short-term and long-term interests encoding across all the users, which is not ideal as users interests are diverse.

\noindent\textbf{Is Quaternion Adversarial training on BPR loss helpful?} We compare our proposed models when training with \emph{BPR} loss (i.e. \emph{QUALE, QUASE (LSTM),} and \emph{QUALSE} models) with our proposed models when training with \emph{QABPR} loss (i.e. \emph{AQUALE}, \emph{AQUASE (LSTM)}, and \emph{AQUALSE}). First, we observe that \emph{AQUASE} boosted \emph{QUASE} performance by a large margin: improving \emph{HIT@100} by 3.2\% and \emph{NDCG@100} by 4.29\% on average in the six datasets. \emph{AQUALE} and \emph{AQUALSE} also improves \emph{QUALE} and \emph{AQUALSE} by 1.92\% and 1.91\% on average of both \emph{HIT@100} and \emph{NDCG@100} over six datasets, respectively. These results show the effectiveness of the adversarial attack on Quaternion representations with our \emph{QABPR} loss. %We note that the improvement on \emph{NDCG} ranking measurement is higher than \emph{HIT} when using \emph{AQBPR} loss is mostly due to the nature of \emph{BPR} loss which aims to ameliorate ranking scores. Additionally, though being effective, \emph{QUALE} is much more simpler than \emph{QUASE} model, leading to a more robust model and a smaller improvement of \emph{AQUALE} on \emph{QUALE}, compared to the enhancement of \emph{AQUASE} on \emph{QUASE}.

%\noindent\textbf{Efficiency of Quaternion representations over real-valued representations?} In section \ref{sec:intro}, we have shown that Quaternion transformation layers reduce 4 times number of needed parameters compared to the real-valued transformations. To further explore, we compare the inference time of \emph{QUALE} vs \emph{AASVD}, and \emph{QUASE} vs \emph{ALSTM}. With a same system and experiment configuration (i.e. Nvidia GeForce GTX 1080 Ti with a batch size of 1000 and embedding size of 64, and test on \emph{Apps for Android} dataset), we observe that due to the paramemeter reduction, \emph{QUALE} takes only 9 seconds/epoch, while \emph{AASVD} takes 12 seconds/epoch. \emph{QUASE} takes 103 seconds/epoch, which is almost 3 times faster than \emph{ALSTM} (307 seconds/epoch). The efficiency is clear in \emph{QUASE} because \emph{QUALE} inherits \emph{ASVD} and requires less Quaternion transformations than the \emph{QUASE}. The running report confirms the efficiency of Quaternion-based models over the corresponding real-valued models.

%\noindent\textbf{How many parameters can we free and how fast is it when using Quaternion representations instead of real-valued representations?}

%%%%%%%%%% ATTENTION ANALYSIS %%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[t]
    \centering
	\begin{subfigure}{0.23\textwidth}
		\centering
		\includegraphics[width=0.48\textwidth]{figs/attention-a-Apps_for_Android-aqsvd.png}
		\includegraphics[width=0.48\textwidth]{figs/attention-a-Apps_for_Android-asvd++.png}
		\vspace{-5pt}
		\caption{QUALE (left) vs AASVD (right). }%($\rho=0.232$) ($\rho=0.216$).}
		\label{fig:attention-apps-aqsvd}
	\end{subfigure}
	\begin{subfigure}{0.23\textwidth}
		\centering
		\includegraphics[width=0.48\textwidth]{figs/attention-a-Apps_for_Android-aqlstm.png}
		\includegraphics[width=0.48\textwidth]{figs/attention-a-Apps_for_Android-lstm++.png}
		\vspace{-5pt}
		\caption{QUASE (left) vs ALSTM (right).}%($\rho=0.148$) ($\rho=0.1$).}
		\label{fig:attention-apps-aqlstm}
	\end{subfigure}
	
    \vspace{-10pt}
    \caption{Comparison of attention scores in our models and in respective real-valued models. Pearson correlation $\rho$ between attention scores and PMI scores are: $\rho_{QUALE}=0.232 > \rho_{AASVD}=0.216$, $\rho_{QUASE}=0.148 > \rho_{ALSTM}=0.1$. }
    \label{fig:attention-analysis}
    \vspace{-10pt}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%\noindent\textbf{Parameter saving?} Our Quaternion-based models share the same number of parameters for user and item embeddings compared to real-valued architecture-alike models, but save 4 times number of parameters used for transformation. For example, the real-valued architecture-alike \emph{ALSTM} needs eight $d\times d$ weight matrices in LSTM cell, and another $d\times d$ weight matrix in Equa~(\ref{equa:q-user-short}), which leads to a total of $9d^2$ parameters. In contrast, our \emph{QUASE} model needs only $9d^2/4$ parameters.






%\noindent\textbf{Sensitivity of our Quaternion-based proposals when varying the embedding size?}

% \textbf{Sensitivity of our Adversarial Quaternion-based proposals when varying the Quaternion adversarial noise magnitude $\epsilon$?}

% \textbf{Sensitivity when varying the $\lambda_{adv}$?} 

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

